Approximate nearest neighbors search without false negatives for $l_2$ for $c>\sqrt{\log\log{n}}$

In this paper, we report progress on answering the open problem presented by Pagh~[14], who considered the nearest neighbor search without false negatives for the Hamming distance. We show new data structures for solving the $c$-approximate nearest neighbors problem without false negatives for Euclidean high dimensional space $\mathcal{R}^d$. These data structures work for any $c = \omega(\sqrt{\log{\log{n}}})$, where $n$ is the number of points in the input set, with poly-logarithmic query time and polynomial preprocessing time. This improves over the known algorithms, which require $c$ to be $\Omega(\sqrt{d})$. This improvement is obtained by applying a sequence of reductions, which are interesting on their own. First, we reduce the problem to $d$ instances of dimension logarithmic in $n$. Next, these instances are reduced to a number of $c$-approximate nearest neighbor search instances in $\big(\mathbb{R}^k\big)^L$ space equipped with metric $m(x,y) = \max_{1 \le i \le L}(\lVert x_i - y_i\rVert_2)$.

==> circle_picture.tex <==
\begin{figure}[ht!]

\centering

\begin{tikzpicture}[scale = 0.3]

\draw[pattern=north east lines] (0,0) circle (2cm);
\draw[dashed] (0,0) circle (3cm);
\draw(0,0) circle (7cm);


\begin{scope}[rotate=315]
    \draw[thick,->] (0,0) -- (2,0) node[anchor=west] {$R$};
\end{scope}
\begin{scope}[rotate=345]
    \draw[thick,->] (0,0) -- (3,0) node[anchor=west] {$\sqrt{\log{\log{d}}} R$};
\end{scope}

\begin{scope}[rotate=285]
    \draw[thick,->] (0,0) -- (7,0) node[anchor=west] {$c R$};
\end{scope}

\node[align=left] at (0,0)   {$q$ \;\;};
\node at (1,1)   {\textbullet $p_1$};
\node at (2,4)   {\textbullet $p_3$};
\node at (-1,-2) {\textbullet $p_2$};
\node at (-7,4) {\textbullet $p_4$};


\end{tikzpicture}
\caption{The presented algorithms guarantee that points in the dashed area ($p_1$) will be reported as neighbors.
    Points within the dotted circle ($p_2$) will be reported as neighbor with high probability.
    Points ($p_3$) within a distance $cR$  might be reported, but not necessarily.
    Points ($p_4$) outside circle $cR$ cannot be reported. 
    }
\label{fig:circle}
\end{figure}


==> conversion_lemma.tex <==
%TO NIE JEST NIGDZIE UZYWANE!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!

Let $\cone$ be a cone measure on the $\sphere$ . As stated in Proposition 3.2 in  \cite{cone}:

\begin{lemma}
Let $d\in \mathbb{N}$, $1 \le p < \infty$, 
and $g_1, \dots, g_d$ 
be independent real-valued random variables that are distributed according to the density
\[f_p(t) = \frac{e^{-|t|^p}}{2\Gamma(1+1/p)}. \]
Consider the random vector $G = (g_1, \dots, g_d)$ and put $Y = G / \dist{G}_p$.
Then $Y$ is independant of $\dist{G}_p$ and has distribution $\cone$.
\end{lemma}

On the other hand, as stated in Theorem 1 in \cite{cone_vol}
\begin{theorem}
Let $d\in \mathbb{N}$, $1 \le p < \infty$, 
and $g_1, \dots, g_d$ 
be independent real-valued random variables that are distributed according to the density $f_p$.
Let $G = (g_1, \dots, g_d)$ be a random vector and put
\[Y = \frac{G}{  (\sum_i g_i^p + Z)^{1/p}},\]
where $Z$ is an exponensioal random variable (i.e. has density $f_1$).
Then $V$ generates  the normalized volume measure on $\ball$, that is, for any measurable $A \subset \Rdspace$,
\[\prob{V\in A} = \frac{vol(A \cap \ball)}{vol(\ball)} \]
\end{theorem}

Let $\gamma_n^{p}$ be a measure induced by 

The $\cone$ measure does coincide with the surface measure only for $d=1,2\infty$.
The following lemma is the generalization of Lemma 2 in \cite{small_ball}

\begin{lemma}
\end{lemma}




